BrainODE: Dynamic Brain Signal Analysis via Graph-Aided Neural Ordinary Differential Equations

Brain network analysis is vital for understanding the neural interactions regarding brain structures and functions, and identifying potential biomarkers for clinical phenotypes. However, widely used brain signals such as Blood Oxygen Level Dependent (BOLD) time series generated from functional Magnetic Resonance Imaging (fMRI) often manifest three challenges: (1) missing values, (2) irregular samples, and (3) sampling misalignment, due to instrumental limitations, impacting downstream brain network analysis and clinical outcome predictions. In this work, we propose a novel model called BrainODE to achieve continuous modeling of dynamic brain signals using Ordinary Differential Equations (ODE). By learning latent initial values and neural ODE functions from irregular time series, BrainODE effectively reconstructs brain signals at any time point, mitigating the aforementioned three data challenges of brain signals altogether. Comprehensive experimental results on real-world neuroimaging datasets demonstrate the superior performance of BrainODE and its capability of addressing the three data challenges.

==> sections/outline.tex <==
\section{Outline}


\subsection{Intro}
(simplyfy the three paragraph)
The importance of brain network analysis (both in application and research). what is fMRI data and what can it do.  

Introduce the pipeline of brain analysis and the importance of preprocessing data and the bad effect of ignoring the existing problem on performance data.

Talks about the problem with current raw BOLD signals and the existing method to solve it. Highlight the shortcoming of these methods and there is a lack of a unified framework for preprocessing the data

Introduce neural ODE (why we use it and its advantage), briefly introduce LG, CG and some related work.

Introduce our proposed unified methods to address problems (a), (b) and (c). Briefly introduce the pipeline and why it can solve the problem

Introduce the motivation and the use of the Spatio graph and temporal graph. Talk about how to construct the two graphs.

Summarizes our contributions
(Background and question, method, experiment(add some num))

Ethical issues

\subsection{Related work}

Graph Neuarl Network (GNN) in Brain Network Analysis

Ordinary Differential Equation (ODE) in Multi-agent Dynamical System Continuous Modeling

\subsection{Method}
(add why design)
Problem definition, highlight the input and output of the model

Model overview.
briefly introduce the component and function of each part in the model. 


Short-Term and Long-Term Time Encoder
why use it ,how use it, result.
Introduce the use of CNN to capture the short Term time information
Introduce the use of self-attention to capture the short Term time information

Spatial Relation and Temporal Relation Learning
(do we need to explain the motivation for using the two graphs again?)
introduce how to construct the two graphs and the use of two graphs.

Generative Model and Decoder
similar to LG.

Training
similar to LG.
(Time complexity)
\subsection{Exp}
RQ1: the improvement of opponent models' and our model's performance with different base models on two datasets.

RQ 2.1: performance on solving missing value task (interpolation and extrapolation task)
performance on solving Time Stamp Alignment and Sample Frequency Unification task
2.2 ablation
2.3 parameter
RQ3: Time 

dataset: abide and abcd are similar to brain network transformer. 
Introduce the simulating dataset.


Opponent Model and Base Model
The opponent model means the model doing similar things to our model in preprocessing data.
The base model means the model that uses the preprocessed data to make predictions.


Metrics: RQ1:similar to brain network transformer.
RQ2,RQ3:similar to LG and CG

Implement details:
talks about the dataset split, the segment of time series. 
optimizer learning rate, epoch num

Detailed analysis of results for RQ1,2,3

For RQ1, our model's improvement is highest with different base models in two datasets.
The analysis has the following part:
briefly analyze the performance of base models before preprocessing
briefly analyze the performance of two datasets before preprocessing
briefly analyze the improvement of different base models and dataset
analyze the improvement of BrainODE and its opponents after preprocessing, highlight why BrainODE's improvement is the highest


For RQ2, our model's MSE is the lowest compared with the opponent models.
The analysis has the following part:
The different performance on two datasets
The different performance in different time length
The different performance between in and ex tasks
The different performance of the different models

For RQ3, our model's MSE is the lowest compared with the opponent models.
similar to RQ2



Ablation study: 
Compare our model with no pos-encoder, temporal graph, spatial graph

Hyperparameter Study:
Draw two images (hidden state size and performance, filter length and performance)

Time Complexity Analysis and Real Running Time Comparison
Give the time complexity of our model and a table of real running time. (do we need to compare the training time?)

Appendix
\subsection{Appendix}
detailed info on datasets

data preparation detail


Implement Details

compare with different ODE solver

other param analysis

software version

% Mention technical part in more details related to our own design, related to brain fmri signals.
% Keep method part to 3 pages
% add time complexity in method
% conclusion: limited clinical insight
% visualize problems and desired outcome in intro
